Helenos: A Realistic Benchmark for Distributed Transactional Memory

Transactional Memory (TM) is an approach to concurrency control that aims to make writing parallel programs both effective and simple. The approach is started in non-distributed multiprocessor systems, but is gaining popularity in distributed systems to synchronize tasks at large scales. Efficiency and scalability are often the key issues in TM research, so performance benchmarks are an important part of it. However, while standard TM benchmarks like the STAMP suite and STMBench7 are available and widely accepted, they do not translate well into distributed systems. Hence, the set of benchmarks usable with distributed TM systems is very limited, and must be padded with microbenchmarks, whose simplicity and artificial nature often makes them uninformative or misleading. Therefore, this paper introduces Helenos, a realistic, complex, and comprehensive distributed TM benchmark based on the problem of the Facebook inbox, an application of the Cassandra distributed store.

==> benchmarks.tex <==
%
\section{Benchmark}
\label{sec:benchmarks}

%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%

